Scaling up Superconducting Quantum Computers with Cryogenic RF-photonics

Today's hundred-qubit quantum computers require a dramatic scale up to millions of qubits to become practical for solving real-world problems. Although a variety of qubit technologies have been demonstrated, scalability remains a major hurdle. Superconducting (SC) qubits are one of the most mature and promising technologies to overcome this challenge. However, these qubits reside in a millikelvin cryogenic dilution fridge, isolating them from thermal and electrical noise. They are controlled by a rack-full of external electronics through extremely complex wiring and cables. Although thousands of qubits can be fabricated on a single chip and cooled down to millikelvin temperatures, scaling up the control and readout electronics remains an elusive goal. This is mainly due to the limited available cooling power in cryogenic systems constraining the wiring capacity and cabling heat load management. In this paper, we focus on scaling up the number of XY-control lines by using cryogenic RF-photonic links. This is one of the major roadblocks to build a thousand qubit superconducting QC. We will first review and study the challenges of state-of-the-art proposed approaches, including cryogenic CMOS and deep-cryogenic photonic methods, to scale up the control interface for SC qubit systems. We will discuss their limitations due to the active power dissipation and passive heat leakage in detail. By analytically modeling the noise sources and thermal budget limits, we will show that our solution can achieve a scale up to a thousand of qubits. Our proposed method can be seamlessly implemented using advanced silicon photonic processes, and the number of required optical fibers can be further reduced by using wavelength division multiplexing (WDM).

==> Extra_Notes.tex <==
%%%% Text that has not been used in the paper ...

The aim of this project is to demonstrate a scalable solution for superconducting QCs to enable the first noisy intermediate-scale quantum (NISQ) processor with over a thousand qubits and realize real-world scale applications. 

to overcome the challenge mentioned above by combining the latest advances in RF-photonics and cryogenic silicon photonics . 

In order to realize the first scalable QC that can support over thousand qubits, we will develop a cryogenic RF-photonic link. 

In doing so, our cryogenic chip can be ultralow power ($<$0.7mW/qubit) as all complex RF blocks are moved to the room-temperature chip thanks to the use of RF-photonic links.




%%%% \section{Noise Requirements}
\label{sec:noise}

In this section, we will introduce the noise requirements for the dilution fridge.

For noise, there are a couple different sources along the interconnect path.
There is noise from any cmos/photonic hardware within these intermediate stages. Additionally, and most importantly, there is also thermal noise. When you keep all your signals at 300K, you have some thermal noise 4kZ*T. This is usually smaller than the signal and not something you have to consider.

When you generate your signal at 300K and are sending it down to 10mK, then you have to start thinking about it. Then, assuming Z is 50ohms at both 300K and at the (MXC) 10mK stage, the thermal noise at the 10mK stage is 30000x larger than it should be. Because the amplitude of the signal being sent to the qubit is small (about -66 dBm), this large thermal noise could overwhelm the signal. To prevent this, attenuation can be added between different stages to decrease the thermal noise. However, then additional considerations to the heat load need to be made.




\begin{figure}[ht]
    \begin{center}
        \includegraphics[width=0.3\textwidth, keepaspectratio]{images/finalboard.PNG}
        \caption
        {
           Do we need this???? Figure With a CMOS amplifier, what are the PMOS and NF limits
        }
        \label{fig:cmosamp}
    \end{center}
\end{figure}
